Reasoning in Large Language Models Through Symbolic Math Word Problems

Large language models (LLMs) have revolutionized NLP by solving downstream tasks with little to no labeled data. Despite their versatile abilities, the larger question of their ability to reason remains ill-understood. This paper addresses reasoning in math word problems (MWPs) by studying symbolic versions of the numeric problems, since a symbolic expression is a "concise explanation" of the numeric answer. We create and use a symbolic version of the SVAMP dataset and find that GPT-3's davinci-002 model also has good zero-shot accuracy on symbolic MWPs. To evaluate the faithfulness of the model's reasoning, we go beyond accuracy and additionally evaluate the alignment between the final answer and the outputted reasoning, which correspond to numeric and symbolic answers respectively for MWPs. We explore a self-prompting approach to encourage the symbolic reasoning to align with the numeric answer, thus equipping the LLM with the ability to provide a concise and verifiable reasoning and making it more interpretable. Surprisingly, self-prompting also improves the symbolic accuracy to be higher than both the numeric and symbolic accuracies, thus providing an ensembling effect. The SVAMP_Sym dataset will be released for future research on symbolic math problems.

==> background.tex <==
\section{Background}
\label{sec:background}






\ns{This section is basically not needed for ACL audience. Can be moved to the appendix}


\input{table_fig/svamp_example}



In this section we describe the basic usage of language models for downstream tasks that leverages their natural language generation abilities.


\subsection{Language Models}
\label{sec:lm}

\ns{This section is not needed for ACL audience.}
Given a sequence of words $(x_1, ..., x_{n})$, an LM is trained to output a distribution over the next word $x_{n+1}$ in the attempt to approximate the distribution $p(x_{n+1} \mid x_1, \dots, x_{n})$.
For instance, for \texttt{prompt} = \texttt{"I went to the caf\'e and ordered a "}, good LM would assign high probability to $p(\texttt{"coffee"} \mid \texttt{prompt})$ but low probability to $p(\texttt{"dolphin"} \mid \texttt{prompt})$.
In general, for any text \texttt{prompt}, an LM can generate a response by sampling one word at a time, until it outputs a pre-specified \texttt{STOP} token:
\begin{align*}
    x_{1} \sim  p&(\cdot \mid \texttt{prompt})\\
    x_{2} \sim  p&(\cdot \mid \texttt{prompt}, x_{1})\\
    &\vdots\\
    x_{n} \sim p(\cdot \mid \texttt{prompt}&, x_{1}, \dots, x_{n-1})\text{ and }x_{n} = \texttt{STOP}
\end{align*}
For a question-answering task, e.g. solving a math word problem, one can provide the question as $\texttt{prompt} = \texttt{"Q: <Question>, A: "}$ and hope that the LM generates some answer to the question.
\Cref{fig:svamp_exmple} shows a concrete example of the output of GPT-3 \citep{brown2020language} can generate for math problems; see \Cref{sec:outputs} for many more examples.
This generation ability of language models can be used for a diverse set of natural language tasks \citep{brown2020language}.




\subsection{Zero-shot and Few-shot Evaluations.}
\label{eq:zero_few_shot}

\ns{Don't need this}

Zero-shot evaluation refers to the case where an LM is directly expected to solve a math problem, without having access to solutions to any problem. Few-shot evaluation first provides the LM with some problems along with solutions, in order to prime it to generate the right answer with a higher likelihood.
Prior work \citep{brown2020language,wei2022chain,kojima2022large} has found that while LMs perform well on many downstream tasks even in the zero-shot setting, often priming the model with a few examples leads to an improvement in the performance.
The prompt for two-shot evaluation would look like \texttt{"Q: <Question\_1>, A: <Answer\_1> Q: <Question\_2>, A: <Answer\_2> Q: <Question\_1>, A:"}.
We evaluate both zero-shot and few-shot settings in \Cref{sec:exps}.






==> prompt.tex <==


